Reinforcement Learning for Agile Active Target Sensing with a UAV

Active target sensing is the task of discovering and classifying an unknown number of targets in an environment and is critical in search-and-rescue missions. This paper develops a deep reinforcement learning approach to plan informative trajectories that increase the likelihood for an uncrewed aerial vehicle (UAV) to discover missing targets. Our approach efficiently (1) explores the environment to discover new targets, (2) exploits its current belief of the target states and incorporates inaccurate sensor models for high-fidelity classification, and (3) generates dynamically feasible trajectories for an agile UAV by employing a motion primitive library. Extensive simulations on randomly generated environments show that our approach is more efficient in discovering and classifying targets than several other baselines. A unique characteristic of our approach, in contrast to heuristic informative path planning approaches, is that it is robust to varying amounts of deviations of the prior belief from the true target distribution, thereby alleviating the challenge of designing heuristics specific to the application conditions.

==> background.tex <==

\subsection{Partially Observable Markov Decision Process}
A POMDP is a tuple  $(\mathcal{S}, \mathcal{A}, \mathcal{T} , \mathcal{O}, R, O, \gamma,d_0)$,
where $\mathcal{S}$, $\mathcal{A}$, $\mathcal{O}$ denote the state space, action space and observation space of the POMDP respectively. $R$, $O$ are the reward and observation
models, $\mathcal{T}$ is a transition dynamics model, $d_0$ is the initial state distribution, and $\gamma$ is the discount factor.
The policy $\pi$ does not have access to the true state $s_t$ and instead has access to an observation $o_t \sim \mathcal{O}(s_t)$.The policy can be stochastic or deterministic (one-hot) distribution over the action space $\mathcal{A}$. The POMDP transitions to the new state according to $s_{t+1} \sim \mathcal{T}(.\;,a_t \sim \pi(o_t),s_t) $ and the objective is to maximize the cumulative expected return from an initial state $s_0 \sim d_0$ and the expected trajectory sampled by unrolling the the policy $\pi$ as follows:

\begin{equation}
J(\pi) = \mathop{\mathbb{E}}_{\substack{s_0 \sim d_0 \; a_t \sim \pi(o_t)\\ o_t \sim \mathcal{O}(s_t) \; s_{t+1} \sim \mathcal{T}(.;a_t,s_t)}} [\sum_{t = 0}^{T}\; \gamma^t \; R(s_t,a_t)] 
\end{equation}


\subsection{Deep Reinforcement Learning}

Deep reinforcement learning aims to maximize the cumulative return $J(\pi)$ under a policy is parameterized by a deep neural network $\theta$ as follows $\pi(o_t;\theta)$.
\begin{equation}
    \theta^* = \mathop{\mathrm{argmax}}_{\theta} \; J(\pi(o_t;\theta))
\end{equation}

The policy is optimized by collecting data from many interactions in the environment. Many algorithms exists for optimizing the returns over the policy parameters \cite{arulkumaran2017deep}. In particular we use the Asynchronous Actor Critic (A3C)for finding a policy over primitives as described in the next section. \cite{mnih2016asynchronous}



==> data/div_performance.tex <==
\definecolor{mBlue}{HTML}{1F77B4}
\definecolor{mDarkBrown}{HTML}{604c38}
\definecolor{mDarkTeal}{HTML}{23373b}
\definecolor{mSteelGray}{HTML}{2B2E34}
\definecolor{mLightBrown}{HTML}{EB811B}
\definecolor{mLightGreen}{HTML}{14B03D}
\definecolor{mDarkRed}{HTML}{a2282f}

\begin{tikzpicture}
	\begin{axis}[
		enlargelimits=true,
		xlabel = {KL-Divergence ($\times 10^{-2}$)},
		ylabel = {Search Performance (\%)},
		legend pos=north east,
        legend cell align=left,
		legend style={font=\tiny},
		height=5cm,
		width=\columnwidth,
		label style={font=\footnotesize},
		tick label style={font=\footnotesize},
		]
		\addplot[
    		only marks,
			mark=square*,
			mark size=1.0pt,
			color=red,
			x filter/.code={\pgfmathparse{\pgfmathresult-0.1}\pgfmathresult},
			error bars/.cd,
            x dir=both, x explicit,
            y dir=both, y explicit]
			table[x=Div,y=RLmean,y error=RLstdev, col sep=comma]
			{results.csv};
		\addplot[
    		only marks,
			mark=triangle*,
			mark size=1.0pt,
			color=mBlue,
			error bars/.cd,
            x dir=both, x explicit,
            y dir=both, y explicit]
			table[x=Div,y=PCmean,y error=PCstdev, col sep=comma]
			{results.csv};
		\addplot[
    		only marks,
			mark=diamond*,
			mark size=1.0pt,
			color=mLightGreen,
			x filter/.code={\pgfmathparse{\pgfmathresult+0.1}\pgfmathresult},
			error bars/.cd,
            x dir=both, x explicit,
            y dir=both, y explicit]
			table[x=Div,y=DPmean,y error=DPstdev, col sep=comma]
			{results.csv};
		 \legend{RL, PC, DP}
	\end{axis}
\end{tikzpicture}


==> data/plot_div_results.tex <==
\definecolor{mBlue}{HTML}{1F77B4}
\definecolor{mDarkBrown}{HTML}{604c38}
\definecolor{mDarkTeal}{HTML}{23373b}
\definecolor{mSteelGray}{HTML}{2B2E34}
\definecolor{mLightBrown}{HTML}{EB811B}
\definecolor{mLightGreen}{HTML}{14B03D}
\definecolor{mDarkRed}{HTML}{a2282f}

\usetikzlibrary{pgfplots.statistics}
    \pgfmathdeclarefunction{fpumod}{2}{%
        \pgfmathfloatdivide{#1}{#2}%
        \pgfmathfloatint{\pgfmathresult}%
        \pgfmathfloatmultiply{\pgfmathresult}{#2}%
        \pgfmathfloatsubtract{#1}{\pgfmathresult}%
        \pgfmathfloatifapproxequalrel{\pgfmathresult}{#2}{\def\pgfmathresult{3.4}}{}%
    }
	\begin{tikzpicture}
	\footnotesize
		\pgfplotsset{
			my boxplot style/.style={
				boxplot,
				solid,
				fill=white,
				mark=*,
				mark size=1.0pt,
				every mark/.append style={
					fill=white,
				},
				},
		}
		\makeatletter
		\pgfplotsset{
			% example copied from the manual
			boxplot/draw/average/.code={%
				\draw[/pgfplots/boxplot/every average/.try]
				\pgfextra
				% do NOT use \draw[mark=*] plot coordinates because
				% boxplots uses the same plot handler to draw its
				% outliers.
				\pgftransformshift{%
					\pgfplotsboxplotpointabbox
					{\pgfplotsboxplotvalue{average}}
					{0.5}%
				}%
				\pgfuseplotmark{\tikz@plot@mark}%
				\endpgfextra
				;
			},
			boxplot/every average/.style={
			/tikz/mark=diamond*,
			},
		}
		\makeatother
		\begin{axis}[
			boxplot,
			boxplot/draw direction=y,
			xtick={0,1,2,3,4,5,6,7},
			xtick={0,1,2,3,4,5,6,7,8},
			xticklabels={0,0.5,1,1.5,2,2.5,3,3.5,4},
			enlarge y limits,
			enlarge x limits=0.04,
			boxplot/average={auto},
			ylabel = {Search Performance (\%)},
			xlabel = {KL Divergence ($\times 10^{-2}$)},
			ylabel near ticks,
			grid=major,
			ymajorgrids=false,
			boxplot={
			draw position={0.2 + floor(\plotnumofactualtype/3) + 0.3*(fpumod(\plotnumofactualtype, 3))},
			box extend=0.2,
			whisker extend=0.1,
			},
			height=5cm,
			width=1.04\columnwidth,
			label style={font=\footnotesize},
			legend entries = {RL, PC, DP-IPP},
			legend to name={legend},
			legend style={font=\tiny},
			name=border
			]
			\addplot[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results025.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results025.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results025.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results075.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results075.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results075.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results125.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results125.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./dat)a/results125.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results175.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results175.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results175.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results225.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results225.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results225.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results275.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results275.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results275.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results325.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results325.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results325.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results375.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results375.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results375.csv};
		\end{axis}
		\node[above right] at (border.south west) {\ref{legend}};
	\end{tikzpicture}


==> data/plot_div_results_bkk.tex <==
\definecolor{mBlue}{HTML}{1F77B4}
\definecolor{mDarkBrown}{HTML}{604c38}
\definecolor{mDarkTeal}{HTML}{23373b}
\definecolor{mSteelGray}{HTML}{2B2E34}
\definecolor{mLightBrown}{HTML}{EB811B}
\definecolor{mLightGreen}{HTML}{14B03D}
\definecolor{mDarkRed}{HTML}{a2282f}

\usetikzlibrary{pgfplots.statistics}
    \pgfmathdeclarefunction{fpumod}{2}{%
        \pgfmathfloatdivide{#1}{#2}%
        \pgfmathfloatint{\pgfmathresult}%
        \pgfmathfloatmultiply{\pgfmathresult}{#2}%
        \pgfmathfloatsubtract{#1}{\pgfmathresult}%
        \pgfmathfloatifapproxequalrel{\pgfmathresult}{#2}{\def\pgfmathresult{3.4}}{}%
    }
	\begin{tikzpicture}
	\centering
	\footnotesize
		\pgfplotsset{
			my boxplot style/.style={
				boxplot,
				solid,
				fill=white,
				mark=*,
				mark size=1.0pt,
				every mark/.append style={
					fill=white,
				},
				},
		}
		\makeatletter
		\pgfplotsset{
			% example copied from the manual
			boxplot/draw/average/.code={%
				\draw[/pgfplots/boxplot/every average/.try]
				\pgfextra
				% do NOT use \draw[mark=*] plot coordinates because
				% boxplots uses the same plot handler to draw its
				% outliers.
				\pgftransformshift{%
					\pgfplotsboxplotpointabbox
					{\pgfplotsboxplotvalue{average}}
					{0.5}%
				}%
				\pgfuseplotmark{\tikz@plot@mark}%
				\endpgfextra
				;
			},
			boxplot/every average/.style={
			/tikz/mark=diamond*,
			},
		}
		\makeatother
		\begin{axis}[
			boxplot,
			boxplot/draw direction=y,
			xtick={0,1,2,3,4,5,6,7,8},
			xticklabels={0,0.5,1,1.5,2,2.5,3,3.5,4},
			enlarge y limits,
			enlarge x limits=0.04,
			restrict x to domain=0:4,
			boxplot/average={auto},
			ylabel = {Search Performance (\%)},
			xlabel = {KL Divergence ($\times 10^{-2}$)},
			ylabel near ticks,
			grid=major,
			ymajorgrids=false,
			boxplot={
			draw position={0.2 + floor(\plotnumofactualtype/3) + 0.3*(fpumod(\plotnumofactualtype, 3))},
			box extend=0.2,
			},
			height=5cm,
			width=1.04\linewidth,
			label style={font=\footnotesize},
			tick style={font=\tiny},
			legend entries = {RL, PC, DP-IPP},
			legend to name={legend},
			legend style={font=\tiny},
			name=border
			]
			\addplot[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results025.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results025.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results025.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results075.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results075.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results075.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results125.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results125.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results125.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results175.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results175.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results175.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results225.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results225.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results225.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results275.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results275.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results275.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results325.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results325.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results325.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results375.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results375.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results375.csv};
		\end{axis}
		\node[above right] at (border.south west) {\ref{legend}};
	\end{tikzpicture}


==> data/plot_div_results_new_v2.tex <==
\definecolor{mBlue}{HTML}{1F77B4}
\definecolor{mDarkBrown}{HTML}{604c38}
\definecolor{mDarkTeal}{HTML}{23373b}
\definecolor{mSteelGray}{HTML}{2B2E34}
\definecolor{mLightBrown}{HTML}{EB811B}
\definecolor{mLightGreen}{HTML}{14B03D}
\definecolor{mDarkRed}{HTML}{a2282f}

\usetikzlibrary{pgfplots.statistics}
    \pgfmathdeclarefunction{fpumod}{2}{%
        \pgfmathfloatdivide{#1}{#2}%
        \pgfmathfloatint{\pgfmathresult}%
        \pgfmathfloatmultiply{\pgfmathresult}{#2}%
        \pgfmathfloatsubtract{#1}{\pgfmathresult}%
        \pgfmathfloatifapproxequalrel{\pgfmathresult}{#2}{\def\pgfmathresult{3.4}}{}%
    }
	\begin{tikzpicture}
	\footnotesize
		\pgfplotsset{
			my boxplot style/.style={
				boxplot,
				solid,
				fill=white,
				mark=*,
				mark size=1.0pt,
				every mark/.append style={
					fill=white,
				},
				},
		}
		\makeatletter
		\pgfplotsset{
			% example copied from the manual
			boxplot/draw/average/.code={%
				\draw[/pgfplots/boxplot/every average/.try]
				\pgfextra
				% do NOT use \draw[mark=*] plot coordinates because
				% boxplots uses the same plot handler to draw its
				% outliers.
				\pgftransformshift{%
					\pgfplotsboxplotpointabbox
					{\pgfplotsboxplotvalue{average}}
					{0.5}%
				}%
				\pgfuseplotmark{\tikz@plot@mark}%
				\endpgfextra
				;
			},
			boxplot/every average/.style={
			/tikz/mark=diamond*,
			},
		}
		\makeatother
		\begin{axis}[
			boxplot,
			boxplot/draw direction=y,
			xtick={0,1,2,3,4,5,6},
			xticklabels={0,0.3,0.6,0.9,1.2,1.5,1.8},
			enlarge y limits,
			enlarge x limits=0.04,
			boxplot/average={auto},
			ylabel = {Search Performance (\%)},
			xlabel = {KL Divergence},
			ylabel near ticks,
			grid=major,
			ymajorgrids=false,
			boxplot={
			draw position={0.2 + floor(\plotnumofactualtype/4) + 0.20*(fpumod(\plotnumofactualtype, 4))},
			box extend=0.2,
			whisker extend=0.1,
			},
			height=5cm,
			width=1.04\columnwidth,
			label style={font=\footnotesize},
			legend entries = {Ours-noLSTM, Ours-LSTM, PC, DP-IPP},
			legend to name={legend},
			legend style={font=\tiny},
			name=border
			]
			\addplot[my boxplot style,draw=mDarkRed]table[y=Ours-noLSTM, col sep=comma]{./data/results0.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=Ours-LSTM, col sep=comma]{./data/results0.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=PC, col sep=comma]{./data/results0.csv};
			\addplot+[my boxplot style,draw=mDarkBrown]table[y=DPIPP, col sep=comma]{./data/results0.csv};
			
    		\addplot+[my boxplot style,draw=mDarkRed]table[y=Ours-noLSTM, col sep=comma]{./data/results1.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=Ours-LSTM, col sep=comma]{./data/results1.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=PC, col sep=comma]{./data/results1.csv};
			\addplot+[my boxplot style,draw=mDarkBrown]table[y=DPIPP, col sep=comma]{./data/results1.csv};
			
			\addplot+[my boxplot style,draw=mDarkRed]table[y=Ours-noLSTM, col sep=comma]{./data/results2.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=Ours-LSTM, col sep=comma]{./data/results2.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=PC, col sep=comma]{./data/results2.csv};
			\addplot+[my boxplot style,draw=mDarkBrown]table[y=DPIPP, col sep=comma]{./data/results2.csv};
			
			
			\addplot+[my boxplot style,draw=mDarkRed]table[y=Ours-noLSTM, col sep=comma]{./data/results3.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=Ours-LSTM, col sep=comma]{./data/results3.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=PC, col sep=comma]{./data/results3.csv};
			\addplot+[my boxplot style,draw=mDarkBrown]table[y=DPIPP, col sep=comma]{./data/results3.csv};
			
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results225.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results225.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results225.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results275.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results275.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results275.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results325.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results325.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results325.csv};
			\addplot+[my boxplot style,draw=mDarkRed]table[y=RL, col sep=comma]{./data/results375.csv};
			\addplot+[my boxplot style,draw=mBlue]table[y=PC, col sep=comma]{./data/results375.csv};
			\addplot+[my boxplot style,draw=mLightGreen]table[y=DP, col sep=comma]{./data/results375.csv};
		\end{axis}
		\node[above right] at (border.south west) {\ref{legend}};
	\end{tikzpicture}

